Capabilities for Better ML Engineering

In spite of machine learning's rapid growth, its engineering support is scattered in many forms, and tends to favor certain engineering stages, stakeholders, and evaluation preferences. We envision a capability-based framework, which uses fine-grained specifications for ML model behaviors to unite existing efforts towards better ML engineering. We use concrete scenarios (model design, debugging, and maintenance) to articulate capabilities' broad applications across various different dimensions, and their impact on building safer, more generalizable and more trustworthy models that reflect human needs. Through preliminary experiments, we show capabilities' potential for reflecting model generalizability, which can provide guidance for ML engineering process. We discuss challenges and opportunities for capabilities' integration into ML engineering.

==> body/6-appendices.tex <==
\section{Experiment Setting}
\label{appendix:experiment}

% We have discussed capabilities' broad applications for ML engineering across different stages, stakeholders, and attributes.
% However, there still exist many challenges in integrating capabilities into ML engineering. 
% We next list challenges and discuss their research opportunities.

\paragraph{Data}
We use the \textsc{Amazon-wilds} dataset~\cite{pmlr-v139-WILDS} for sentiment analysis.
The dataset consists of Amazon reviews of many different categories and their ratings.
We select the \textsc{Home-and-kitchen} category for training and ten other categories for evaluation. 
In domain adaptation, the \textsc{Home-and-kitchen} category would be referred to as source domain, while the other categories are target domains. 
Following previous work in domain adaptation~\cite{blitzer-etal-2007-biographies}, we convert ratings to binary labels (positive when >3, negative when <3) and sample a balanced dataset for each category (domain).

\paragraph{Model}
% We select two model architectures for our evaluation: LSTM and BERT~\cite{bhargava2021generalization, DBLP:journals/corr/abs-1908-08962}.
% We trained 200 LSTM models and 
To obtain a series of models with different accuracy, we fine-tuned a pre-trained BERT model~\cite{bhargava2021generalization, DBLP:journals/corr/abs-1908-08962} 100 times on different random seeds.

\paragraph{Method}
Our goal is to observe the correlations between model accuracy across source domain and target domains,
as well as how extra information (e.g., accuracy on capability test suites) would affect the correlations.

We first use a linear model to compute the correlations of accuracy between source domain and target domains, without any extra variables.
We then introduce three sets of variables to the linear model:

\begin{enumerate}
    \item \textit{Capability test suite accuracy}: we first selected eight capabilities for sentiment analysis based on an existing study~\cite{barnes-etal-2019-sentiment}. We instantiated these capabilities by slicing the source domain dataset on their corresponding keywords (see Tab.~\ref{tab:cap-inst}).
    We computed the models' accuracy on the capability test suites and removed five of them due to collinearity. 
    The final capabilities we used are \textit{shifter}, \textit{modality}, and \textit{comparative}.
    \item \textit{Random subset accuracy}: we selected three random subsets from the source dataset. These subsets are of the same size as the three capability test suites. We computed the models' accuracy on the random subsets.
    \item \textit{Noisy accuracy}:  we added random Gaussian noise to the models' validation accuracy.
    % \item \textit{Long text subset's accuracy}: we selected texts longer than 150 tokens from source dataset and computed models' accuracy on the slice.
\end{enumerate}

For the last two settings, we repeated the process on 100 different random seeds and averaged their results.

We then fit the linear model with these extra variables for each setting.
We looked at adjusted $R^2$ to see whether the model has a better fit (i.e., whether these extra variables help predict out-of-distribution accuracy). 
\footnote{$R^2$ represents the proportion of the variance that could be explained by input variables. 
Higher $R^2$ implies a better fit of the linear model and higher predictive power of input variables.
We used adjusted $R^2$ to compensate for the effect of extra degrees of freedom. It only increases if the new variable enhances the model above what would be obtained by chance.}
We also performed \textsc{ANOVA} testing to see whether the improvement is statistically significant. 

To understand the relation between capability predictiveness and distribution distance, we followed the method from previous work~\cite{blitzer-etal-2007-biographies} to compute a proxy $\mathcal{A}$-distance between different domains.

% \section{Experiment Results}
% We found that capabilities better help predict model generalization compared to all other baselines.
% The linear model's adjusted $R^2$ increases (statistically significantly) in 50\% domains with extra variables from capabilities.
% In contrast, the best baseline (random subsets) only increases adjusted $R^2$ in 20\% domains on average (see Fig.~\ref{fig:improvement} for details).

% For finetuned BERT models, that adjustd $R^2$ increases significantly in 5 out of 10 casese

% We found that different capabilities add different information for prediction.
% Some capabilities (e.g., \textit{negation}) produce too many test cases, which leads to an uninformative distribution close to the original dataset.
% Different capabilities could also augment each other: 
% \textit{shifter} improves predictive power in 2 cases, but adding \textit{modality} further increases predictive power in 4 cases.


% We found that capabilities' predictiveness correlates with distribution distance (see Fig.~\ref{fig:distance}). 
% The further the domain is, the better capabilities could help predict generalization.
% We hypothesize that this might be due to the fact that if a target domain is too close to the source domain,
% there is little room left for improvement.


==> body/_dep_-4-experiment.tex <==
\section{Preliminary Results}


% We have discussed capabilities' broad applications for ML engineering across different stages, stakeholders, and attributes.
% However, there still exist many challenges in integrating capabilities into ML engineering. 
% We next list challenges and discuss their research opportunities.
We conducted an exploratory experiment to evaluate how useful capabilities are for model generalization,
which is the focus in our model maintenance scenario and important for many other scenarios as well.

The key finding is that generic capabilities are already helpful in predicting how well models could generalize to out-of-distribution data.
This provides further evidence that capabilities could be useful beyond the explored use cases in testing and debugging.
We next describe the experiment settings and results in detail.



\paragraph{Data}
We use the \textsc{Amazon-wilds} dataset~\cite{pmlr-v139-koh21a} for sentiment analysis.
The dataset consists of Amazon reviews of many different categories and their ratings.
We select \textsc{Home-and-kitchen} category for training and 10 other categories for evaluation. 
In domain adaptation, the \textsc{Home-and-kitchen} category would be referred to as source domain, while other categories are target domains. 
Following previous works in domain adaptation~\cite{blitzer-etal-2007-biographies}, we convert ratings to binary labels (positive when >3, negative when <3) and sample a balanced dataset for each category (domain).

\paragraph{Model}
% We select two model architectures for our evaluation: LSTM and BERT~\cite{bhargava2021generalization, DBLP:journals/corr/abs-1908-08962}.
% We trained 200 LSTM models and 
To obtain a series of models with different accuracies, we finetuned a pre-trained BERT model~\cite{bhargava2021generalization, DBLP:journals/corr/abs-1908-08962} 100 times on different random seeds.

\paragraph{Method}
Our goal is to observe the correlations between models' accuracies across source domain and target domains,
as well as how extra information (e.g., accuracies on capability test suites) would affect the correlations.

We first use a linear model to compute the correlations of accuracies between source domain and target domains, without any extra variables.
We then introduce three sets of variables to the linear model:

\begin{enumerate}[(a)]
    \item \textit{Capability test suites' accuracies}: we first selected 8 capabilities for sentiment analysis based on an existing study~\cite{barnes-etal-2019-sentiment}. We instantiated these capabilities by slicing the source domain dataset on their corresponding keywords (see Appendix~\ref{sec:cap-select} for details). We computed models' accuracies on the capability tests and removed five of them to avoid collinearity~\cite{}. 
    % The details of this process could be found in the Appendix~\ref{sec:cap-select}.
    \item \textit{Random subsets' accuracies}: we selected three random subsets from source dataset. These subsets are of the same size of three capability test suites. We computed models' accuracies on the random subsets.
    \item \textit{Noisy accuracies}:  we added random Gaussian noise to models' validation accuracies.
    % \item \textit{Long text subset's accuracies}: we selected texts longer than 150 tokens from source dataset and computed models' accuracies on the slice.
\end{enumerate}

For the settings in (b) and (c), we repeat the process on 100 different random seeds and average their results.

We then fit the linear model with these extra variables for each setting.
We looked at adjusted $R^2$ to see whether the model has a better fit (i.e., whether these extra variables help predict out-of-distribution scores). 
\footnote{$R^2$ represents the proportion of the variance that could be explained by input variables. 
Higher $R^2$ implies a better fit of the linear model and higher predictive power of input variables.
We used adjusted $R^2$ to compensate the effect of extra degrees of freedom. It only increases if the new variable enhances the model above what would be obtained by chance.}
We also performed \textsc{ANOVA} testing to see whether the improvement is statistically significant. 

\paragraph{Results}
We found that capabilities better help predict model generalization compared to all other baselines.
The linear model's adjusted $R^2$ increases (statistically significantly) in 50\% domains with extra variables from capabilities.
In contrast, the best baseline (random subsets) only increases adjusted $R^2$ in 20\% domains on average (see Fig.~\ref{fig:improvement} for details).

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/plot-improvement}
    \caption{Capabilities better help predict model generalization.}
    \label{fig:improvement}
\end{figure}
% For finetuned BERT models, that adjustd $R^2$ increases significantly in 5 out of 10 casese


\sherry{
% so do you want this to be a separate section or a sub-section?

% And I think we can write it to be:

% 1. We use some preliminary results to show the feasibility of using capabilities for essential ML engineering steps

% 2. We focus on generalization because it's related to multiple scenarios (see comments in table 1 caption)

3. We show capability tests:

3a. is predictive to model generalizability -> would help in debugging, doing better on capabilites actually mean (v.s. checklist only shows capabilities can expose model problems but didnt build the relation of better capablity -> better generalization)

3b. their predictiveness correlates with dataset distance -> would be useful for quality assurance for downstream deployment in particular domains

3c. Multiple capabilities add more information -> communication \& negotiation among multiple stakeholders

4. However, there are:

4a. uninformative capabilities that would just be removed because they overlap too much with dev set 

4b. Task specific vs. task agnostic capabilities

-> capability identification is important and instantiation is also important

-> Next section talks more about challenges and opportunities
}

